Ultracold Neutral Plasmas

Ultracold neutral plasmas, formed by photoionizing laser-cooled atoms near the ionization threshold, have electron temperatures in the 1-1000 kelvin range and ion temperatures from tens of millikelvin to a few kelvin. They represent a new frontier in the study of neutral plasmas, which traditionally deals with much hotter systems, but they also blur the boundaries of plasma, atomic, condensed matter, and low temperature physics. Modelling these plasmas challenges computational techniques and theories of non-equilibrium systems, so the field has attracted great interest from the theoretical and computational physics communities. By varying laser intensities and wavelengths it is possible to accurately set the initial plasma density and energy, and charged-particle-detection and optical diagnostics allow precise measurements for comparison with theoretical predictions. Recent experiments using optical probes demonstrated that ions in the plasma equilibrate in a strongly coupled fluid phase. Strongly coupled plasmas, in which the electrical interaction energy between charged particles exceeds the average kinetic energy, reverse the traditional energy hierarchy underlying basic plasma concepts such as Debye screening and hydrodynamics. Equilibration in this regime is of particular interest because it involves the establishment of spatial correlations between particles, and it connects to the physics of the interiors of gas-giant planets and inertial confinement fusion devices.

==> intro-jm-old.tex <==
In a conventional neutral plasma, ions and electrons are created
from atoms and molecules by ionizing collisions between particles.
Because a typical ionization potential is on the order of an
electronvolt, most neutral plasmas have temperatures of thousands of
kelvin or more. Plasma physics in this regime encompasses a wealth
of fascinating fundamental  phenomena such as collective modes,
instabilities, and transport mechanisms, and it can contribute to
important applications such as lighting technologies, plasma
processing, and the pursuit of fusion energy.
%It  and also enables important applications such as
% lighting, plasma processing, and the pursuit of fusion energy.
Our
understanding and corresponding theories of these plasmas %systems
 are based on the dominance  of thermal (kinetic) energy
%an assumption that thermal
over interaction (potential) energy, but how do plasmas behave at
lower temperatures where this might not be the case?
%
%and how do we understand them at lower temperatures where kinetic
%energy does not dominate potential energy in the plasma?

%Until recently, before ultracold plasmas were realized, this question
%was very difficult to answer since plasmas  in the parameter regime
%of  strong coupling were hardly accessible exerimentally.
%And even if they could be created or were naturally given, their very
%nature has precluded precise measurement of their evolution in time
%etc.  (see figure Pauli xxx), discuss  CCP etc. (jm) \JMe

\begin{table}
  \centering
  \caption{Typical parameters of neutral plasmas.}\label{nuetralplasmastable}
\end{table}


It is possible to address this question with experimental,
theoretical, and computational studies of ultracold neutral plasmas
\cite{kkb99}, which are formed by photoionizing laser-cooled atoms
near the ionization threshold. These systems  have electron
temperatures ranging from 1-1000\,K and ion temperatures of around
1\,K, and they stretch the boundaries of traditional neutral plasma
physics. While providing access to a new regime, they have also
proven to be clean and simple systems that form an excellent testing
ground for basic plasma theory, and they elucidate physics found
across a much wider spectrum of plasma energy and density.




The clearest distinguishing feature of ultracold neutral plasmas is
that particles can be in or near the strongly coupled regime
\cite{ich82}.  In strongly coupled plasmas the Coulomb interaction
energy between charged particles exceeds the average kinetic energy,
which is quantified by the Coulomb coupling parameter
\begin{equation}\label{coulombcouplingdefinition}
\Gamma= e^2 / [4\pi \varepsilon_0 a k_B T],
\end{equation}
where $a=[3/(4 \pi \rho)]^{1/3}$ is the Wigner-Seitz radius
characterizing the separation between particles in a plasma of
density $\rho$ and temperature $T$. $\Gamma>1$ reverses the
traditional energy hierarchy that underlies our normal understanding
of plasmas based on concepts such as Debye screening and
hydrodynamics. Strongly coupled plasmas exist in dense astrophysical
systems \cite{vho91}, matter irradiated with intense laser fields
\cite{nmg98,sht00,rem05}, colloidal or dusty plasmas of highly
charged macroscopic particles \cite{mtk99,hol00b}, and non-neutral
trapped ion plasmas  that are laser cooled until they freeze into
Wigner crystals \cite{mbh99}.  Strong coupling is manifested through
the presence of spatial correlations between particles, which can be
important for the equilibration and collective dynamics of the
system.  Optical probes \cite{scg04,cdd05} demonstrated that ions in
an ultracold neutral plasma can be strongly coupled.  Electrons seem
to remain just outside of this regime because the rate of
recombination of electrons and ions to form neutral particles
diverges rapidly as the electron temperature drops.

Immediately after the creation of an ultracold neutral plasma
through photoionization, the system is far from equilibrium, and
most research in the field has focused on the equilibration process.
Theoretical and computational work
\cite{mur01,kon02prl,kon02,mck02,rha02,rha03,tya00} has  identified
 processes that heat the plasma.
%Because the Coulomb
%potential energy is relatively large,
For plasmas in or near the strongly coupled regime, where the
potential energy is comparable to or exceeds the thermal energy,
 excess potential energy arising from a random
distribution of ions \cite{mur01} or electrons \cite{kon02prl} is
converted to thermal energy. This is called \emph{disorder-induced
heating}. Another important heating mechanism is \emph{Three-body
recombination} (TBR), in which an ion and two electrons collide to
form an energetic electron and an excited neutral atom.   The TBR
rate varies with temperature as $T^{-9/2}$ \cite{mke69}, and at low
temperatures it can become the fastest process in the plasma.
%For a cold plasma one is of course interested
%to minimize TBR. However,
TBR is a crucial process for the formation of cold antihydrogen
through positron-antiproton recombination \cite{aab02,gbo02}.
Conditions in these anti-matter plasmas are similar to ultracold
neutral plasmas except a large magnetic field is usually present to
contain the particles. Surprisingly, recombination in ultracold
neutral plasmas also has similarities to stellar dynamics in
globular clusters \cite{cvz05}.





The study of collective modes has proven to be a rich area of
research, originally motivated by the possibility of observing
modification of the mode structure due to strong coupling
\cite{kgm93}.  Electron plasma oscillations \cite{kkb00,bsp03} and
Tonks-Dattner modes \cite{fzr06} have served as probes of plasma
dynamics and represent interesting fundamental problems in their own
right.

There is great similarity between the dynamics of ultracold neutral plasmas
and equilibration of plasmas created by irradiation
of solid \cite{ckz00,skh00} and thin film targets
 \cite{hbc00,mgf00,bwp01,msp02,hkp02,asa03,kss04,fsk05,rfb05}
 , clusters \cite{dts97},
 and gas jets \cite{sbn99,kcn99} by
 fast pulse lasers.
The excellent characterization and control available
 in the ultracold
regime imply that significant scientific contributions can be made
by
 exploiting this connection. And in
  ultracold,  low density samples,  timescales for
  physical processes become longer, which facilitates their observation.
Studies of ion equilibration
 have revealed oscillations of the ion kinetic
 energy \cite{csl04,ppa05conf,ppr05prl,mur06PRL}
 that are a fundamental characteristic of equilibration of strongly
 coupled systems.
 Expansion of a plasma into the surrounding vacuum may be directly
 observed with excellent spatial and temporal resolution
 in ultracold systems \cite{kkb00,rha03,ppr04,cdd05}.
This phenomenon is important in fast-pulse experiments,
especially in the context of the
 generation of high energy particles
 \cite{ckz00,skh00,hbc00,mgf00,bwp01,msp02,hkp02,asa03,kss04,fsk05,rfb05,dts97,sbn99,kcn99},
 inertial-confinement fusion
 experiments \cite{lin95}, and x-ray lasers \cite{dai02}.
 %Significant theoretical effort
% (e.g. \cite{ssc87,bku98,dse98,kby03,ccb05,mor05}).

 %****It would be better for somebody else to fill in these details**
 High energy-density and strongly coupled plasmas are often difficult to
 describe theoretically because
 of the importance of many-body interactions, and these problems are often best
 addressed with computational techniques. Many body interactions are
 also important in ultracold
 neutral plasmas, and computational physicists have
 made significant contributions to the understanding of these system
 by applying techniques usually used for high energy-density systems
 \cite{kon02,mck02}. Ultracold
 plasmas have motivated the development and application
 of numerical recipes to describe the presence of spatial
 correlations between the ions \cite{ppr04}
and the evolution
 of electrons and ions on very different timescales \cite{kon02}.
 Again, the excellent experimental control and
 diagnostics available imply that these computational results can be
 tested with great precision in ultracold systems.


The review is structured such that  Sections
\ref{sectionexperimentalaspects} and \ref{sectiontheoreticalaspects}
provide the experimental and theoretical basis that allows one to
understand and manipulate ultracold neutral plasmas. The main
Section \ref{sectionphysprocess} of the review describes the
physical processes which take place in an ultracold neutral plasma
from the time it is created until it expands into the surrounding
vacuum.
%This section  may be read directly without Sections
%\ref{sectionexperimentalaspects} and
%\ref{sectiontheoreticalaspects}, although their knowledge is
%necessary for a deeper understanding of the processes.
 In Section \ref{sectionachievingstringcoupling}, we discuss
 proposals and prospects for achieving very strong coupling of the
 plasma -- in some sense the ``holy grail'' of ultracold plasma physics.
 We conclude with Section \ref{sectionfuture} by discussing some possible
 future directions of this relatively young research field.

